Optimistic Rates for Learning with a Smooth Loss

We establish an excess risk bound of O(H R_n^2 + R_n \sqrt{H L*}) for empirical risk minimization with an H-smooth loss function and a hypothesis class with Rademacher complexity R_n, where L* is the best risk achievable by the hypothesis class. For typical hypothesis classes where R_n = \sqrt{R/n}, this translates to a learning rate of O(RH/n) in the separable (L*=0) case and O(RH/n + \sqrt{L^* RH/n}) more generally. We also provide similar guarantees for online and stochastic convex optimization with a smooth non-negative objective.

==> temp.tex <==
\appendix
\section{Technical Proofs}

\begin{proof}[{\bf Proof of Lemma \ref{lem:key}}]
In order to prove Lemma \ref{lem:key}, we actually move from
Rademacher complexity to covering numbers, use smoothness and Lemma
\ref{lemma:smooth} to obtain an $r$-dependent cover of the empirically
restricted class, and then return to the Rademacher complexity.  

Before we proceed, recall the following definitions of covering numbers and fat shattering dimension.
For any $\epsilon >0$ and function class $\mathcal{F} \subset \mathbb{R}^{\mathcal{Z}}$: 
\begin{description}
\item[ ] \vspace{-0.1in} The $L_2$ covering number $\mathcal{N}_2\left(\mathcal{F},\epsilon, n\right)$ is the supremum over samples $z_1,\ldots,z_n$ of the size of a minimal cover $\mathcal{C}_\epsilon$ such that 
$\forall f \in \mathcal{F}$, $\exists f_\epsilon \in
\mathcal{C}_\epsilon$ s.t.~$\sqrt{\frac{1}{n}
  \sum_{i=1}^n (f(z_i) - f_\epsilon(z_i))^2} \le
\epsilon$.\\
\item[ ] \vspace{-0.15in} The $L_\infty$ covering number $\mathcal{N}_\infty\left(\mathcal{F},\epsilon, n\right)$  is the supremum over samples $z_1,\ldots,z_n$ of the size of a minimal cover $\mathcal{C}_\epsilon$ such that
$\forall f \in \mathcal{F}$,  $\exists f_\epsilon \in
\mathcal{C}_\epsilon$ s.t.~$ \max_{i \in [n]} |f(z_i) - f_\epsilon(z_i)| \le
\epsilon$.\\
\item[ ] \vspace{-0.15in} The fat-shattering dimension
  $\mathrm{fat}_{\epsilon}(\mathcal{F})$ at scale $\epsilon$ is the
  maximum number of points $\epsilon$-shattered by $\mathcal{F}$ (see
  e.g.~\cite{Mendelson02}).
\end{description}


\vspace{-0.2in}
\paragraph{Bounding $\hRad_n(\cL_\phi(r))$ in terms of
  $\mathcal{N}_2(\cL_\phi(r))$}
Dudley's integral bound lets us bound the Rademacher complexity of a
class in terms of its empirical $L_2$ covering number. Here we use a
more refined version of Dudley's integral bound due to Mendelson
\cite{Mendelson02} and more explicitly stated in \cite{SrebroSr10} and
included for completeness as Lemma \ref{lem:cover} in the Appendix:
\begin{align}\label{eq:dud}
  \hRad_n(\cL_\phi(r))\le \inf_{\alpha > 0}\left\{ 4 \alpha + 10
    \int_{\alpha}^{\sqrt{b r}}
    \sqrt{\frac{\mathcal{N}_2\left(\cL_\phi(r),\epsilon,
          n\right)}{n}} d \epsilon \right\}
\end{align}

\paragraph{Bounding $\mathcal{N}_2(\cL_\phi(r))$ in terms of
  $\mathcal{N}_{\infty}(\mathcal{H})$}
In the Appendix we show that a corollary of Lemma \ref{lemma:smooth}
is that for a non-negative $H$-smooth $f(\cdot)$ we have $\left(f(t) -
  f(r)\right)^2 \le 6 H ( f(t) + f(r) )  (t - r)^2$ (Lemma
\ref{lem:smoothbnd}).  Using this inequality, for any sample
$(x_1,y_1),\ldots,(x_n,y_n)$:
\begin{align*}
\sqrt{\frac{1}{n} \sum_{i=1}^n (\phi(h(z_i),z_i) - \phi(h_\epsilon(z_i),z_i))^2}  & \le \sqrt{\frac{6 H}{n} \sum_{i=1}^n \left( \phi(h(z_i),z_i)  +  \phi(h_\epsilon(z_i),z_i)\right) (h(z_i) - h_\epsilon(z_i))^2} \\ 
& \le \sqrt{\frac{6 H}{n} \sum_{i=1}^n \left( \phi(h(z_i),z_i)  +  \phi(h_\epsilon(z_i),z_i)\right) } \sqrt{\max_{i \in [n]} (h(z_i) - h_\epsilon(z_i))^2}\\
& \le \sqrt{12 H  r}\ \max_{i \in [n]}| h(z_i) - h_\epsilon(z_i)|
\end{align*}
That is, an empirical $L_{\infty}$ cover of $\left\{h \in \H : \hL(h)
  \le r \right\}$ at radius $\epsilon/\sqrt{12 H r}$ is also an
empirical $L_2$ cover of $\cL_\phi(r)$ at radius $\epsilon$, and we
can conclude that:
\begin{equation}\label{eq:N2Ninf}
\mathcal{N}_2\left(\cL_\phi(r),\epsilon, n\right) \le \mathcal{N}_\infty\left(\left\{h \in \H : \hL(h) \le r\right\},\frac{\epsilon}{\sqrt{12 H r}}, n\right) \le \mathcal{N}_\infty\left(\H,\frac{\epsilon}{\sqrt{12 H r}}, n\right)
\end{equation}

\paragraph{Bounding $\mathcal{N}_{\infty}(\mathcal{H})$ in terms of $\hRad_n(\H)$}
  Note that for any $\epsilon > \Rad_n(\mathcal{H})$, by Lemma \ref{lem:fatrad}, $\mathrm{fat}_\epsilon \le n$. Hence the $L_{\infty}$ covering number at scale $\epsilon/\sqrt{12 H r}$  can be bounded
in terms of the fat shattering dimension at
that scale using Lemma \ref{lem:covfat} \cite{Mendelson02} as:
\begin{equation}\label{eq:NinfFat}
\mathcal{N}_\infty\left(\H,\frac{\epsilon}{\sqrt{12 H r}}, n\right) \le \left(\frac{2 e n \ \sqrt{12 H r} B }{\epsilon\ \mathrm{fat}_\frac{\epsilon}{\sqrt{12 H r}}(\mathcal{H}) }\right)^{\mathrm{fat}_\frac{\epsilon}{\sqrt{12 H r}}(\mathcal{H})}~.
\end{equation}

Hence by Equation \eqref{eq:dud} we have:
\begin{align}
\hRad_n(\cL_\phi(r)) & \le  4 \sqrt{12 H r} \Rad_n(\mathcal{H}) + 10 \int_{\sqrt{12 H r} \Rad_n(\mathcal{H})}^{\sqrt{b r}} \sqrt{\frac{\mathrm{fat}_\frac{\epsilon}{\sqrt{12 H r}}(\mathcal{H}) \log\left(\frac{2 e n \ \sqrt{12 H r} B }{\epsilon \mathrm{fat}_\frac{\epsilon}{\sqrt{12 H r}}(\mathcal{H}) }\right)}{n}} d \epsilon 
\intertext{after a change of integration variable:}
& \le  4 \sqrt{12 H r}\Rad_n(\mathcal{H}) + 10 \sqrt{12 H r} \int_{\Rad_n(\mathcal{H})}^{\sqrt{b/12 H}} \sqrt{\frac{\mathrm{fat}_\epsilon(\mathcal{H}) \log\left(\frac{2 e n \  B }{\epsilon \mathrm{fat}_\epsilon(\mathcal{H}) }\right)}{n}} d \epsilon \\
& \le  4 \sqrt{12 H r}\Rad_n(\mathcal{H}) + 10 \sqrt{12 H r} \int_{\Rad_n(\mathcal{H})}^{\sqrt{b/12 H}} \sqrt{\frac{\mathrm{fat}_\epsilon(\mathcal{H}) \log\left(\frac{2 e  B }{\epsilon  }\right)}{n}} d \epsilon \notag \\
& ~~~~~~~~~~~~~~~~~~~~~~~~+ 10 \sqrt{12 H r} \int_{\Rad_n(\mathcal{H})}^{\sqrt{b/12 H}} \sqrt{\frac{\mathrm{fat}_\epsilon(\mathcal{H}) \log\left(\frac{n}{\mathrm{fat}_\epsilon(\mathcal{H}) }\right)}{n}} d \epsilon  \label{eq:3term}
\end{align}
We now bound the second term in the sum above. To this end note that for any $\epsilon \ge \Rad_n(\mathcal{H})$, bounding the fat-shattering dimension in terms of the  Rademacher complexity (Lemma \ref{lem:fatrad}) we get:
\begin{align}\label{eq:2ndterm}
10 \sqrt{12 H r} \int_{\Rad_n(\mathcal{H})}^{\sqrt{b/12 H}} \sqrt{\frac{\mathrm{fat}_\epsilon(\mathcal{H}) \log\left(\frac{2 e  B }{\epsilon  }\right)}{n}} d \epsilon & \le  10 \sqrt{12 H r}\ \Rad_n(\mathcal{H}) \int_{\Rad_n(\mathcal{H})}^{\sqrt{b/12 H}} \frac{\sqrt{\log\left(\frac{2 e B}{\epsilon}\right)}}{\epsilon} d \epsilon \notag \\
& \le  10 \sqrt{12 H r}\ \Rad_n(\mathcal{H}) \left[ -\frac{2}{3} \log^{3/2}\left(\frac{2 e B}{\epsilon}\right)\right]_{\Rad_n(\mathcal{H})}^{\sqrt{b/12 H}}  \notag \\
& \le \frac{20}{3} \sqrt{12 H r}\ \Rad_n(\mathcal{H}) \left(\log^{3/2}\left(\frac{2 e B}{\Rad_n(\mathcal{H})}\right) -  \log^{3/2}\left(\sqrt{\frac{24 e H B^2}{b}}\right) \right) \notag \\
& \le \frac{20}{3} \sqrt{12 H r}\  \log^{3/2}\left(\frac{2 e B}{\Rad_n(\mathcal{H})}\right)  \Rad_n(\mathcal{H})
\end{align}
Now we move to the third term of Equation \ref{eq:3term}, we further split this integral into three parts as :
\begin{align}
 \int_{\Rad_n(\mathcal{H})}^{\sqrt{b/12 H}} \sqrt{\frac{\mathrm{fat}_\epsilon(\mathcal{H}) \log\left(\frac{n}{\mathrm{fat}_\epsilon(\mathcal{H}) }\right)}{n}} d \epsilon & \le  \int_{\Rad_n(\mathcal{H})}^{\gamma} \sqrt{\frac{\mathrm{fat}_\epsilon(\mathcal{H}) \log\left(\frac{n}{\mathrm{fat}_\epsilon(\mathcal{H}) }\right)}{n}} d \epsilon + \int_{\gamma}^{\theta} \sqrt{\frac{\mathrm{fat}_\epsilon(\mathcal{H}) \log\left(\frac{n}{\mathrm{fat}_\epsilon(\mathcal{H}) }\right)}{n}} d \epsilon \notag \\
 & ~~~~~ + \int_{\theta}^{\sqrt{b/12 H}} \sqrt{\frac{\mathrm{fat}_\epsilon(\mathcal{H}) \log\left(\frac{n}{\mathrm{fat}_\epsilon(\mathcal{H}) }\right)}{n}} d \epsilon \notag 
\intertext{Now let $\theta$ be such that $\mathrm{fat}_\theta > n/e$, so that for all $\epsilon > \theta$, $\log(n/\mathrm{fat}_\epsilon) \le 1$. Hence,}
& \le  \int_{\Rad_n(\mathcal{H})}^{\gamma} \sqrt{\frac{\mathrm{fat}_\epsilon(\mathcal{H}) \log\left(\frac{n}{\mathrm{fat}_\epsilon(\mathcal{H}) }\right)}{n}} d \epsilon + \int_{\gamma}^{\theta} \sqrt{\frac{\mathrm{fat}_\epsilon(\mathcal{H}) \log\left(\frac{n}{\mathrm{fat}_\epsilon(\mathcal{H}) }\right)}{n}} d \epsilon \notag \\
 & ~~~~~ + \int_{\theta}^{\sqrt{b/12 H}} \sqrt{\frac{\mathrm{fat}_\epsilon(\mathcal{H}) }{n}} d \epsilon \notag 
\intertext{Now to handle the second term in the integral note that in the range $d \in [1,n/e]$, the function $d \log\left(\frac{n}{d}\right)$ is monotonically increasing in $d$ and so in the range of $\epsilon \in [\gamma,\theta]$, $\mathrm{fat}_\epsilon \log\left(\frac{n}{\mathrm{fat}_\epsilon} \right) \le \mathrm{fat}_\gamma \log\left(\frac{n}{\mathrm{fat}_\gamma} \right)$. Thus we have that }
& \le  \int_{\Rad_n(\mathcal{H})}^{\gamma} \sqrt{\frac{\mathrm{fat}_\epsilon(\mathcal{H}) \log\left(\frac{n}{\mathrm{fat}_\epsilon(\mathcal{H}) }\right)}{n}} d \epsilon + \int_{\gamma}^{\theta} \sqrt{\frac{\mathrm{fat}_\gamma(\mathcal{H}) \log\left(\frac{n}{\mathrm{fat}_\gamma(\mathcal{H}) }\right)}{n}} d \epsilon \notag \\
 & ~~~~~ + \int_{\theta}^{\sqrt{b/12 H}} \sqrt{\frac{\mathrm{fat}_\epsilon(\mathcal{H}) }{n}} d \epsilon \notag 
\intertext{Further since for all $\epsilon \in [\Rad_n(\mathcal{H}), \gamma]$ $\mathrm{fat}_\epsilon \le \mathrm{fat}_\gamma$ we have that}
& \le  \int_{\Rad_n(\mathcal{H})}^{\gamma} \sqrt{\frac{\mathrm{fat}_\epsilon(\mathcal{H}) \log\left(\frac{n}{\mathrm{fat}_\gamma(\mathcal{H}) }\right)}{n}} d \epsilon + \int_{\gamma}^{\theta} \sqrt{\frac{\mathrm{fat}_\gamma(\mathcal{H}) \log\left(\frac{n}{\mathrm{fat}_\gamma(\mathcal{H}) }\right)}{n}} d \epsilon \notag \\
 & ~~~~~ + \int_{\theta}^{\sqrt{b/12 H}} \sqrt{\frac{\mathrm{fat}_\epsilon(\mathcal{H}) }{n}} d \epsilon \notag
\intertext{Since all three integrals above are in the range such that $\epsilon > \Rad_n(\mathcal{H})$,  bounding the fat-shattering dimension in terms of the  Rademacher complexity (Lemma \ref{lem:fatrad}) in the first and third integrals :}
& \le  \Rad_n(\mathcal{H})\int_{\Rad_n(\mathcal{H})}^{\gamma} \frac{\sqrt{\log\left(\frac{n}{\mathrm{fat}_\gamma(\mathcal{H}) }\right)}}{\epsilon} d \epsilon + \int_{\gamma}^{\theta} \sqrt{\frac{\mathrm{fat}_\gamma(\mathcal{H}) \log\left(\frac{n}{\mathrm{fat}_\gamma(\mathcal{H}) }\right)}{n}} d \epsilon \notag \\
 & ~~~~~ + \Rad_n(\mathcal{H}) \int_{\theta}^{\sqrt{b/12 H}} \frac{1}{\epsilon} d \epsilon \notag \\
 & \le  \Rad_n(\mathcal{H})\sqrt{\log\left(\frac{n}{\mathrm{fat}_\gamma(\mathcal{H}) }\right)} \log\left(\frac{1}{\Rad_n(\mathcal{H})}\right) + \sqrt{\frac{\mathrm{fat}_\gamma(\mathcal{H}) \log\left(\frac{n}{\mathrm{fat}_\gamma(\mathcal{H}) }\right)}{n}} \left(\gamma - \theta\right) \notag \\
 & ~~~~~ + \Rad_n(\mathcal{H}) \log\left(\frac{1}{\theta}\right)\notag\\
  & \le  \Rad_n(\mathcal{H})\sqrt{\log\left(\frac{n}{\mathrm{fat}_\gamma(\mathcal{H}) }\right)} \log\left(\frac{1}{\Rad_n(\mathcal{H})}\right) + \sqrt{\frac{\mathrm{fat}_\gamma(\mathcal{H}) \log\left(\frac{n}{\mathrm{fat}_\gamma(\mathcal{H}) }\right)}{n}} \sqrt{\frac{b}{12 H}} \notag \\
 & ~~~~~ + \Rad_n(\mathcal{H}) \log\left(\frac{1}{\Rad_n(\mathcal{H})}\right)\notag 
 \intertext{where in the last inequality we used the fact that $\gamma - \theta \le \sqrt{b/12 H}$ (integral range) and that $\theta \ge \Rad_n(\mathcal{H})$. Picking $\gamma$ to be such that $\mathrm{fat}_\gamma = 12 H n \Rad_n^2(\mathcal{H})/ b $ we conclude that}
  & \le  \Rad_n(\mathcal{H})\sqrt{\log\left(\frac{b}{12 H \Rad^2_n(\mathcal{H}) }\right)} \log\left(\frac{1}{\Rad_n(\mathcal{H})}\right) + \Rad_n(\mathcal{H}) \sqrt{\log\left(\frac{b}{12 H \Rad^2_n(\mathcal{H}) }\right)} \notag \\
 & ~~~~~ + \Rad_n(\mathcal{H}) \log\left(\frac{1}{\Rad_n(\mathcal{H})}\right) \notag\\
 & \le 3\ \Rad_n(\mathcal{H}) \log^{3/2}\left(\frac{2 e B}{\Rad_n(\mathcal{H})}\right)
\end{align}
Hence plugging back the above and Equation \eqref{eq:2ndterm} back in Equation \eqref{eq:3term} we conclude that
\begin{align}\label{eq:removingB}
\hRad_n(\cL_\phi(r)) & \le  4 \sqrt{12 H r}\Rad_n(\mathcal{H}) + 7 \sqrt{12 H r} \Rad_n(\mathcal{H}) \log^{3/2}\left(\frac{2 e B}{\Rad_n(\mathcal{H})}\right) + 30 \sqrt{12 H r} \Rad_n(\mathcal{H}) \log^{3/2}\left(\frac{2 e B}{\Rad_n(\mathcal{H})}\right) \notag \\
& \le 41 \sqrt{12 H r} \Rad_n(\mathcal{H}) \log^{3/2}\left(\frac{2 e B}{\Rad_n(\mathcal{H})}\right)
\end{align}
Now by definition of rademacher complexity we have,
\begin{align*}
\hRad_n(\H) & = \sup_{x_1,\ldots , x_n \in \X} \Es{\sigma \sim \text{Unif}(\{\pm 1\}^n)}{\sup_{h \in \H} \frac{1}{n} \left|\sum_{i=1}^n  h(x_i) \sigma_i \right|}\\
& \ge \sup_{x \in \X} \Es{\sigma \sim \text{Unif}(\{\pm 1\}^n)}{\sup_{h \in \H} \frac{1}{n} \left|\sum_{i=1}^n  h(x) \sigma_i \right|}\\
& = \left(\sup_{x \in \X}\sup_{h \in \H} |h(x)|\right) \  \left(\Es{\sigma \sim \text{Unif}(\{\pm 1\}^n)}{ \frac{1}{n} \left|\sum_{i=1}^n \sigma_i\right|}\right)\\
& = B\ \Es{\sigma \sim \text{Unif}(\{\pm 1\}^n)}{ \frac{1}{n} \left|\sum_{i=1}^n \sigma_i\right|} \ge \frac{B}{\sqrt{2n}}
\end{align*}
where the last step is due to Kintchine's inequality (see Eg. page 364 of \cite{CesaBianchiLu06}). Thus we see that $\frac{2 e B}{\Rad_n(\mathcal{H} }\le 8 \sqrt{n}$. Plugging this in Equation \ref{eq:removingB} we conclude that
\begin{align*}
\hRad_n(\cL_\phi(r)) &  \le 21 \sqrt{6 H r}\ \log^{\frac{3}{2}}\left(64\ n\right) \ \Rad_n(\mathcal{H})
\end{align*}
\end{proof}






